Spatially Attentive Output Layer for Image Classification

Most convolutional neural networks (CNNs) for image classification use a global average pooling (GAP) followed by a fully-connected (FC) layer for output logits. However, this spatial aggregation procedure inherently restricts the utilization of location-specific information at the output layer, although this spatial information can be beneficial for classification. In this paper, we propose a novel spatial output layer on top of the existing convolutional feature maps to explicitly exploit the location-specific output information. In specific, given the spatial feature maps, we replace the previous GAP-FC layer with a spatially attentive output layer (SAOL) by employing a attention mask on spatial logits. The proposed location-specific attention selectively aggregates spatial logits within a target region, which leads to not only the performance improvement but also spatially interpretable outputs. Moreover, the proposed SAOL also permits to fully exploit location-specific self-supervision as well as self-distillation to enhance the generalization ability during training. The proposed SAOL with self-supervision and self-distillation can be easily plugged into existing CNNs. Experimental results on various classification tasks with representative architectures show consistent performance improvements by SAOL at almost the same computational cost.

==> figures/fig_wsol.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\usepackage{changepage,threeparttable}
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}

\begin{table*}[tp]\center

\begin{tabular}{c c c c c | c c c c}
 
\rotatebox[origin=c]{90}{Image} & \includegraphics[scale=0.20]{figures/samples/cub/original/0000_0000_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/original/0000_0003_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/original/0001_0006_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/original/0001_0009_0_falsepositive.jpg}
& \includegraphics[scale=0.20]{figures/samples/imagenet/original/0305_0017_0_truepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/original/0873_0024_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/original/1217_0028_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/original/0526_0022_0_falsepositive.jpg} \\
\rotatebox[origin=cc]{90}{GradCam} & \includegraphics[scale=0.20]{figures/samples/cub/gradcam/0000_0000_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/gradcam/0000_0003_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/gradcam/0001_0006_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/gradcam/0001_0009_0_falsepositive.jpg}
& \includegraphics[scale=0.20]{figures/samples/imagenet/gradcam/0305_0017_0_truepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/gradcam/0873_0024_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/gradcam/1217_0028_0_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/gradcam/0526_0022_0_falsepositive.jpg} \\
\rotatebox[origin=c]{90}{ASOL (Ours)}& \includegraphics[scale=0.20]{figures/samples/cub/our_merge/0000_0000_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/our_merge/0000_0003_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/our_merge/0001_0006_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/cub/our_merge/0001_0009_falsepositive.jpg}
& \includegraphics[scale=0.20]{figures/samples/imagenet/our_merge/0305_0017_truepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/our_merge/0873_0024_falsepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/our_merge/1217_0028_truepositive.jpg} & \includegraphics[scale=0.20]{figures/samples/imagenet/our_merge/0526_0022_truepositive.jpg} \\
 & \multicolumn{4}{c}{CUB-200-2011} & \multicolumn{4}{c}{ImageNet}
 
\end{tabular}

\caption{Comparison with GradCam method. Our method can locate entire objects region to imporve localication performance.}\label{tab:exp-wsol}

\label{fig:comaprision_attention}

\end{table*}


==> tables/ab-attention.tex <==
\begin{table}[H]\centering

\begin{tabular}{l | c | c}\toprule
Model &SAOL &w/o attention \\\midrule
ResNet-50           &77.04 / 93.53 &77.02 / 93.26 \\
ResNet-101          &78.54 / 94.23 &78.50 / 94.06 \\
ResNet-101 + CutMix &80.37 / 94.92 &80.51 / 94.79 \\
\bottomrule

\end{tabular}
\caption{Performance comparison on ImageNet according to whether to use the attention.}\label{tab:ab-attention}

\end{table}

